Interpreting Complex Regression Models

Interpretation of a machine learning induced models is critical for feature engineering, debugging, and, arguably, compliance. Yet, best of breed machine learning models tend to be very complex. This paper presents a method for model interpretation which has the main benefit that the simple interpretations it provides are always grounded in actual sets of learning examples. The method is validated on the task of interpreting a complex regression model in the context of both an academic problem -- predicting the year in which a song was recorded and an industrial one -- predicting mail user churn.

==> algorithm-impl.tex <==
\section{The Algorithm Implementation}

Our implementation of Algorithm~\ref{alg:finalalg} was through the parallel distributed framework of MapReduce. We choose \emph{t}-test as our dissimilarity measurement. For completeness we include the definition of the $2$-sample Student's \emph{t}-test~\cite{TTest}: 
%TODO- check if necessary Both metrics are calculated on two samples. In both cases we remove outliers before the metric is calculated: $10\%$ highest and $10\%$ lowest values are removed from every sample. 

\begin{definition}
%We recall the definition of the (student) 2-sample T-Test we use. 
Given two samples from distributions $\Lcal_1$, and $\Lcal_2$. For $i\in \{1,2\}$, let $\mu_i,  \sigma_i, n_i$ denote the $\Lcal_i$ sample average, standard deviation, and number of elements, respectively.
The (student) $2$-sample t-test is defined to be 
\[ \frac{\mu_1-\mu_2}{\sqrt{\frac{\sigma_1^2}{n_1} + \frac{\sigma_2^2}{n_2} }} \]
\end{definition}

For the implementation of the \emph{t}-test evaluation we used a limited buffer to 
collect the sampled examples from the tested segment and from its complement segment (restricting the sample size to the buffer size used). The following experiment examined the dependence of the algorithm stabilizability as a function of the buffer size. 
For this, the algorithm was applied to generate the top 30 explanatory  features (i.e. features that have segments that were chosen to be at the final top segments group). For statistical significance, for each buffer size, we execute this process 10 times. Then, we compute the average Jaccard similarity between every pair of features set from the 10 executions. 
Figure~\ref{fig:jaccard} present the resulting graph when applied this process on the second use case dataset, with buffers size that  were chosen to be powers of $10$. For the rest of the experimental results (in both use cases) we use a buffer of size $10$K, which received a high Jaccard similarity of $0.871$. 


\begin{figure}[htbp!]
\includegraphics[width=0.45\textwidth]{figs-mail/jaccard_data_standardScale.pdf}
\caption{Jaccard similarity coefficient per buffer size.}\label{fig:jaccard}
 %\vspace{-0.1in}
\end{figure}



==> related.tex <==
\section{RELATED WORK}
One way by which a prediction can be interpreted is using \emph{sensitivity analysis} \cite{saltelli2000sensitivity}. I.e.,  small variations can be introduced to the features of the example and their effect on the prediction can be measured. The main problem with sensitivity analysis is that it requires an understanding of the features. Specifically, the meaning and legitimacy of "small" changes differ between the features. For instance, what might be a "small" change in a gender feature? In a recent paper, Tolomei et al. \cite{tolomei2017interpretable}  address this problem by making use of naturally occurring variations in feature values among the learning examples. Still, their method is not immune to improbable combinations of features.% such as gender and age. 

Ribeiro at el. \cite{RibeiroSG16} suggested a different approach to model interpretation. They describe an algorithm called LIME which identifies regions in the feature space in which classification can be approximated with a linear model. Since a linear model is considered interpretable, the combination of a region division and a linear model is a good explanation. Like previous work, LIME suffers the disadvantage that it is not at all certain that the variation required to change the prediction occurs in reality.

